A Formal Hierarchy of RNN Architectures

We develop a formal hierarchy of the expressive capacity of RNN architectures. The hierarchy is based on two formal properties: space complexity, which measures the RNN's memory, and rational recurrence, defined as whether the recurrent update can be described by a weighted finite-state machine. We place several RNN variants within this hierarchy. For example, we prove the LSTM is not rational, which formally separates it from the related QRNN (Bradbury et al., 2016). We also show how these models' expressive capacity is expanded by stacking multiple layers or composing them with different pooling functions. Our results build on the theory of "saturated" RNNs (Merrill, 2019). While formally extending these findings to unsaturated RNNs is left to future work, we hypothesize that the practical learnable capacity of unsaturated RNNs obeys a similar hierarchy. Experimental findings from training unsaturated networks on formal languages support this conjecture.

==> closure.tex <==
\section{Closure Properties} \label{sec:closure}

We remind the reader that we use $\mathrm{R}$ to denote the set of rational series.

\begin{lemma} \label{thm:add-closure}
    $\mathrm{R}$ is closed under addition; \textit{i.e.} for all $f, g \in \mathrm{R}$, if
    \begin{equation*}
        h(x) = f(x) + g(x) ,
    \end{equation*}
    then $h \in \mathrm{R}$.
\end{lemma}

\begin{proof}
Given a WFAs $A_f$ and $A_g$ computing $f$ and $g$ respectively, we create a new WFA $A'$ by merging the graphs for the two machines (the resulting graph for $A'$ has two independent components). The score $A'[x]$ is the sum of of paths through $A_f$ and the paths through $A_g$. By construction, this is $f(x) + g(x)$.
\end{proof}

\begin{lemma}
    $\mathrm{R}$ is closed under scalar multiplication; \textit{i.e.} for all $f \in \mathrm{R}$ and $w \in \mathbb{Q}$, if
    \begin{equation*}
        g(x) = w f(x) ,
    \end{equation*}
    then $g \in \mathrm{R}$.
\end{lemma}

\begin{proof}
Given a machine $A_f$, we create $A'$ to compute $g$ by multiplying each acceptance weight in $A_f$ by $w$.
\end{proof}

\begin{lemma}
$\mathrm{R}$ is closed under adding a constant; \textit{i.e.} for all $f \in \mathrm{R}$, if
\begin{equation}
    h(x) = f(x) + b ,
\end{equation}
\noindent then $h \in \mathrm{R}$.
\end{lemma}

\begin{proof}
We construct a trivial WFA with one state to compute $b$. Then we apply \autoref{thm:add-closure}.
\end{proof}

An interesting consequence of these results is that rational series are closed under linear transformation.

\begin{lemma}
For all rational series $\bv f : \Sigma^* \rightarrow \mathbb{Q}^k$, as well as $\bv w \in \mathbb{Q}^k$ and $b \in \mathbb{Q}$, the following function $g$ is in R:
\begin{equation*}
    g(x) = \bv w \cdot \bv f(x) + b .
\end{equation*}
\end{lemma}

% \subsection{Restricted CMs}

% We define a slight generalization of the $(\Sigma \times Q)$-restricted CMs. We allow the additive term in the counter update to be any rational value. We call this a rational CM. Note that it is clearly still RR.

% \WM{Might want to introduce the counter machines this way from the get-go.}

% We prove a similar closure result for the fuzzy CMs. Let $\bv f : \Sigma^* \rightarrow \mathbb{Z}^k$ be a function computable by a fuzzy CM.

% \begin{lemma}
% If $f$ is computable by a fuzzy CM, then
% $g(x) = w f(x)$ is computable by a fuzzy CM.
% \end{lemma}

% \begin{proof}
% Replace each update operation $\pm m$ with $\pm wm$.
% \end{proof}

% \begin{lemma}
% If $f$ and $g$ are computable by a fuzzy CM, then
% $h(x) = f(x) + g(x)$ is computable by a fuzzy CM.
% \end{lemma}

% \begin{proof}
% Let $M_f$ and $M_g$ be counter machines computing $f$ and $g$ respectively. We define a new machine $M'$ that simulates 
% \end{proof}

% \begin{lemma}
% Let $\bv f : \Sigma^* \rightarrow \mathbb{Z}^k$ be a function computable by $(\Sigma \times Q)$-restricted CMs. Then the following function is also computable by a $1$-counter $(\Sigma \times Q)$-restricted CM:
% \begin{equation*}
%     g(x) = \bv w \cdot \bv f(x) .
% \end{equation*}
% \end{lemma}
